IsoBench: Benchmarking Multimodal Foundation Models on Isomorphic Representations

Current foundation models exhibit impressive capabilities when prompted either with text only or with both image and text inputs. But do their capabilities change depending on the input modality? In this work, we propose $\textbf{IsoBench}$, a benchmark dataset containing problems from four major areas: math, science, algorithms, and games. Each example is presented with multiple $\textbf{isomorphic representations}$ of inputs, such as visual, textual, and mathematical presentations. IsoBench provides fine-grained feedback to diagnose performance gaps caused by the form of the representation. Across various foundation models, we observe that on the same problem, models have a consistent preference towards textual representations. Most prominently, when evaluated on all IsoBench problems, Claude-3 Opus performs 28.7 points worse when provided with images instead of text; similarly, GPT-4 Turbo is 18.7 points worse and Gemini Pro is 14.9 points worse. Finally, we present two prompting techniques, $\textit{IsoCombination}$ and $\textit{IsoScratchPad}$, which improve model performance by considering combinations of, and translations between, different input representations.

==> sections/results/graph/connectivity.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c | C{0.15\linewidth} | C{0.15\linewidth} | C{0.15\linewidth}}
    \toprule
        \multirow{2}*{Model} &  \multicolumn{3}{c}{Representation}\\
        \cmidrule{2-4}
         &  Image &  Math & Text \\
         \midrule
         GPT-4 Turbo &  78.22 &  79.33 & 95.11\\
         GPT-3.5 Turbo & -- &  50.66 & 75.77\\
         Gemini Pro & 50.22 & 50.00 & 70.88\\
         PaLM-2 (\texttt{text-bison}) & -- & 55.78 &  83.11\\
         Reka Flash & & &\\
         LLaMa-2 (\texttt{llama-2-7b-chat}) & -- & 50.00 & 50.00 \\
         LLaVA-1.5 (\texttt{llava-1.5-13b}) & 50.00 & -- & -- \\
 \bottomrule
    \end{tabular}
    \caption{Benchmark on models abilities to solve \textbf{graph connectivity} problems across three input representations.}
    \label{tab:graph_connectivity}
\end{table}

==> sections/results/graph/isomorphism.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c | C{0.15\linewidth} | C{0.15\linewidth}}
    \toprule
        \multirow{2}*{Model} &  \multicolumn{2}{c}{Representation}\\
        \cmidrule{2-3}
         &  Image &  Math  \\
         \midrule
         GPT-4 Turbo & 57.81 & 62.50 \\
         GPT-3.5 Turbo & -- & 50.00 \\
         Gemini Pro & 50.00 & 70.31 \\
         PaLM-2 (\texttt{text-bison}) & -- & 50.00 \\
         Reka Flash & & \\
         LLaMa-2 (\texttt{llama-2-7b-chat}) & -- & 50.00 \\
         LLaVA-1.5 (\texttt{llava-1.5-13b}) &  & --  \\
 \bottomrule
    \end{tabular}
    \caption{Benchmark on models abilities to solve \textbf{graph isomorphism} problems across two input representations.}
    \label{tab:graph_isomorphism}
\end{table}

==> sections/results/graph/maxflow.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c | C{0.15\linewidth} | C{0.15\linewidth} | C{0.15\linewidth}}
    \toprule
        \multirow{2}*{Model} &  \multicolumn{3}{c}{Representation}\\
        \cmidrule{2-4}
         &  Image &  Math & Text \\
         \midrule
         GPT-4 Turbo &  18 & 18  & 35 \\
         GPT-3.5 Turbo & -- & 14  & 10 \\
         Gemini Pro & 10 & 15 & 11 \\
         PaLM-2 (\texttt{text-bison}) & -- & 19 & 22  \\
         Reka Flash & & &\\
         LLaMa-2 (\texttt{llama-2-7b-chat}) & -- &  8& 10 \\
         LLaVA-1.5 (\texttt{llava-1.5-13b}) & 9  & -- & -- \\
 \bottomrule
    \end{tabular}
    \caption{Benchmark on models abilities to solve \textbf{maximum flow} problems across three input representations.}
    \label{tab:maxflow}
\end{table}


==> sections/teaser_old.tex <==
\titlehook{
\begin{center}
    \ifcolmfinal
    \vspace{-12mm}
    \else
    \vspace{-6mm}
    \fi
    
    \centering
    \captionsetup{type=figure}
    \includegraphics[width=1.04\linewidth]{figures/IsoBench-Teaser.pdf}
    \vspace{-5mm}
    \captionof{figure}{\footnotesize \textbf{Do multimodal foundation models treat every modality equally?} In this example, a model is provided with either an {\color{gblue}image} representation or a {\color{gred}text} representation \textit{isomorphic} to the {\color{gblue}image}, where the {\color{gyellow}instructions} are kept identical. Surprisingly, multimodal foundation models like GPT-4 often give different responses for these isomorphic inputs (\textit{e.g.}, in the figure above, only the response to the {\color{gred}text} representation is correct).
    In \textbf{IsoBench}, we scale such examples into four major domains (\textit{Math}, \textit{Science}, \textit{Algorithms}, \textit{Games}) and find
    a consistent preference towards {\color{gred}text} across many popular multimodal foundation models.
    % that the preference towards {\color{gred}text} is \textit{universal} across multimodal foundation models.
    }
    \label{fig:isobench-teaser}
    \ifcolmfinal
    \vspace{-4mm}
    \fi
\end{center}%
}
